Structural price model for electricity coupled markets

We propose a new structural model that can compute the electricity spot and forward prices in two coupled markets with limited interconnection and multiple fuels. We choose a structural approach in order to represent some key characteristics of electricity spot prices such as their link to fuel prices, consumption level and production fleet. With this model, explicit formulas are also available for forward prices and other derivatives. We give some illustrative results of the behaviour of spot and forward prices, and of the values of transmission rights.

==> abrege.tex <==
% TEX 7(ascii) bits
%
% ABREGE.tex
% LaTeX document
% Author: J.I. 
% Date  : Juillet 1996
%
% Raccourcis d'expressions tr\`es usit\'ees
%
% Derniere modif le 10-07-96
%

% Raccourci pour \XS
\def\XS{\xspace}

%%%%%%%%%%%%%%%%%%% Pour definir nouvelle commande de changement de taille
\RequirePackage{ifthen}
\RequirePackage{calc}

\newcommand{\taille}[1][\scad]{%
\ifthenelse{#1 = -5}{}{}%
\ifthenelse{#1 = -4}{\tiny}{}%
\ifthenelse{#1 = -3}{\scriptsize}{}%
\ifthenelse{#1 = -2}{\footnotesize}{}%
\ifthenelse{#1 = -1}{\small}{}%
\ifthenelse{#1 = 0}{\normalsize}{}%
\ifthenelse{#1 = 1}{\large}{}%
\ifthenelse{#1 = 2}{\Large}{}%
\ifthenelse{#1 = 3}{\LARGE}{}%
\ifthenelse{#1 = 4}{\huge}{}%
\ifthenelse{#1 = 5}{\Huge}{}}

\newboolean{@serif}
\setboolean{@serif}{true}
\def\scad{-5} % scadefaultsize

\newcounter{taille}
\newcommand{\sca}[2][\scad]{\setcounter{taille}{#1}%
  \ifthenelse{\boolean{@serif}}
  {{\taille[\thetaille]\textsc{#2}}}
  {\setcounter{taille}{\value{taille}-1}{\uppercase{\taille[\thetaille]#2}}}}

% Mise en commentaire rapide !
\def\rem#1{}                    % rem{bla bla bla}

% References automatiquement entre parenthese
\def\reff#1{\XS(\ref{#1})}
\def\refs#1{section~\ref{#1}}
\def\refS#1{Section~\ref{#1}}

\newcommand{\clearemptydoublepage}{\newpage{\pagestyle{empty}\cleardoublepage}}  
% Num�ro (pour biblio)
\def\numero{n�}
\def\Numero{N�}

% Majuscules
\def\UP#1{\uppercase{#1}}       % majuscules
\def\up#1{\uppercase{#1}}       % majuscules

% Liste des abreges
\def\adhoc{\textit{ad hoc}\XS}
\def\apost{\textit{a posteriori}\XS}
\def\Apost{\textit{A posteriori}\XS}
\def\APost{\textit{A Posteriori}\XS}
\def\post{\textit{posterior}\XS}
\def\Post{\textit{Posterior}\XS}
\def\afortio{\textit{a fortiori}\XS}
\def\Afortio{\textit{A fortiori}\XS}
\def\aprio{\textit{a priori}\XS}
\def\Aprio{\textit{A priori}\XS}
\def\Cad{C'est-\`a-dire\XS}
\def\cad{c'est-\`a-dire\XS}
\def\coeur{c{\oe}ur\XS}
\def\cf{\textit{cf.}\XS}
\def\cv{\textit{curriculum vit\ae}\XS}
\def\Cv{\textit{Curriculum vit\ae}\XS}
\def\CV{\textit{Curriculum Vit\ae}\XS}
\def\eg{\textit{e.g.,}\XS}
\def\etal{\textit{et al.}\XS}
\def\etc{\textit{etc}\XS}
\def\etcoll{{\textit et coll.}\XS}
\def\idem{\textit{idem}\XS}
\def\ie{\textit{i.e.,}\XS}
\def\IFF{\textit{if and only if}\XS}
\def\iid{i.i.d.\XS}
\def\infine{\textit{in fine}\XS}
\def\insit{\textit{in situ}\XS}
\def\inviv{\textit{in vivo}\XS}
\def\oeuvre{{\oe}uvre\XS}
\def\oeuvres{{\oe}uvres\XS}
\def\oeil{{\oe}il\XS}
\def\recto{\textit{recto}\XS}
\def\Toeplitz{T{\oe}plitz\XS}
\def\vav{vis-\`a-vis\XS}
\def\via{\textit{via}\XS}
\def\vic{\textit{vice-versa}\XS}
\def\verso{\textit{verso}\XS}
%\def\vitae{\textit{vit\ae}\XS}
\def\vs{\textit{vs}\XS}
\def\versus{\textit{versus}\XS}
\def\ssi{\textit{si et seulement si}\XS}
\def\strsen{\textit{stricto sensu}\XS}
\def\wrt{w.r.t.\XS}

\def\ier{$^{\text{\small er}}$\XS}
\def\iere{$^{\text{\small re}}$\XS}
\def\ieme{$^{\text{\small e}}$\XS}

\def\primo{\ensuremath{1^{\oD}}\XS}
\def\secundo{\ensuremath{2^{\oD}}\XS}
\def\tertio{\ensuremath{3^{\oD}}\XS}
\def\quatro{\ensuremath{4^{\oD}}\XS}


\newcommand{\art}[1][\scad]{\sca[#1]{art}\XS}
\newcommand{\cnd}[1][\scad]{\sca[#1]{cnd}\XS}
\newcommand{\ndt}[1][\scad]{\sca[#1]{ndt}\XS}
\newcommand{\gnc}[1][\scad]{\sca[#1]{gnc}\XS}
\newcommand{\mfa}[1][\scad]{\sca[#1]{mfa}\XS}
\newcommand{\map}[1][\scad]{\sca[#1]{map}\XS}

\newcommand{\icm}[1][\scad]{\sca[#1]{icm}\XS}
\newcommand{\icd}[1][\scad]{\sca[#1]{icd}\XS}
\newcommand{\rsb}[1][\scad]{\sca[#1]{rsb}\XS}
\newcommand{\snr}[1][\scad]{\sca[#1]{snr}\XS}

\newcommand{\dess}[1][\scad]{\sca[#1]{dess}\XS}
\newcommand{\dea}[1][\scad]{\sca[#1]{dea}\XS}
\newcommand{\deug}[1][\scad]{\sca[#1]{deug}\XS}
\newcommand{\deust}[1][\scad]{\sca[#1]{deust}\XS}
\newcommand{\iut}[1][\scad]{\sca[#1]{iut}\XS}
\newcommand{\iup}[1][\scad]{\sca[#1]{iup}\XS}

\newcommand{\eea}[1][\scad]{\sca[#1]{eea}\XS}
\def\EEA{\'Electronique \'Electrotechnique Automatique\XS}
\newcommand{\ats}[1][\scad]{\sca[#1]{ats}\XS}
\def\ATS{Automatique et Traitement du Signal\XS}

\newcommand{\te}[1][\scad]{\sca[#1]{te}\XS}
\def\TE{travaux d'�tudes\XS}
\newcommand{\td}[1][\scad]{\sca[#1]{td}\XS}
\def\TD{travaux dirig�s\XS}
\newcommand{\tp}[1][\scad]{\sca[#1]{tp}\XS}
\def\TP{travaux pratiques\XS}
%\newcommand{\tdao}[1][\scad]{\sca[#1]{tdao}\XS}
\def\TDAO{travaux dirig�s assist�s sur ordinateur\XS}
\newcommand{\tdao}[1][\scad]{\sca[#1]{tdao}\XS}
\def\ts{traitement du signal\XS}
\def\TS{Traitement du Signal\XS}

\newcommand{\gbm}[1][\scad]{\sca[#1]{gbm}\XS}
\newcommand{\irmf}[1][\scad]{\sca[#1]{irm-f}\XS}
\newcommand{\irm}[1][\scad]{\sca[#1]{irm}\XS}
\newcommand{\rmn}[1][\scad]{\sca[#1]{rmn}\XS}
\newcommand{\eeg}[1][\scad]{\sca[#1]{eeg}\XS}
\newcommand{\meg}[1][\scad]{\sca[#1]{meg}\XS}

\newcommand{\pc}[1][\scad]{\sca[#1]{pc}\XS}
% Operating Systemes 
\newcommand{\linux}[1][\scad]{\sca[#1]{Linux}\XS}
\newcommand{\unix}[1][\scad]{\sca[#1]{Unix}\XS}
\newcommand{\msdos}[1][\scad]{\sca[#1]{msdos}\XS}
\newcommand{\sunos}[1][\scad]{\sca[#1]{Sunos}\XS}
\newcommand{\hupux}[1][\scad]{\sca[#1]{hp-ux}\XS}
\newcommand{\vms}[1][\scad]{\sca[#1]{vms}\XS}
\newcommand{\solaris}[1][\scad]{\sca[#1]{Solaris}\XS}
\newcommand{\winnt}[1][\scad]{\sca[#1]{Windows-nt}\XS}
\newcommand{\vmware}[1][\scad]{\sca[#1]{vmware}\XS}
\newcommand{\win}[1][\scad]{\sca[#1]{Windows}\XS}

% Calcul scientifique
\newcommand{\labview}[1][\scad]{\sca[#1]{Labview}\XS}
\newcommand{\matlab}[1][\scad]{\sca[#1]{Matlab}\XS}
\newcommand{\maple}[1][\scad]{\sca[#1]{Maple}\XS}
\newcommand{\mathe}[1][\scad]{\sca[#1]{Mathematica}\XS}
\newcommand{\idl}[1][\scad]{\sca[#1]{Idl}\XS}

% langages
\newcommand{\cmex}[1][\scad]{\sca[#1]{Cmex}\XS}
\newcommand{\pascal}[1][\scad]{\sca[#1]{Pascal}\XS}
\newcommand{\java}[1][\scad]{\sca[#1]{Java}\XS}
\newcommand{\lisp}[1][\scad]{\sca[#1]{Lisp}\XS}
\newcommand{\forts}[1][\scad]{\sca[#1]{Fortran}{\footnotesize 77}\XS}
\newcommand{\fortq}[1][\scad]{\sca[#1]{Fortran}{\footnotesize 90}\XS}
\newcommand{\ada}[1][\scad]{\sca[#1]{Ada}\XS}
\newcommand{\eiffel}[1][\scad]{\sca[#1]{Eiffel}\XS}
\newcommand{\tcsh}[1][\scad]{\sca[#1]{tcsh}\XS}
\newcommand{\bash}[1][\scad]{\sca[#1]{bash}\XS}
\newcommand{\lgc}[1][\scad]{\sca[#1]{C}\XS}
\newcommand{\cpp}[1][\scad]{\sca[#1]{C}{\footnotesize ++}\XS}

\def\crec{charg� de recherches\XS}
\def\Crec{Charg� de recherches\XS}
\def\dr{directeur de recherches\XS}
\def\Dr{Directeur de recherches\XS}


% congres
\newcommand{\gretsi}[1][\scad]{\sca[#1]{gretsi}\XS}
\newcommand{\maxent}[1][\scad]{\sca[#1]{maxent}\XS}
\newcommand{\icip}[1][\scad]{\sca[#1]{icip}\XS}
\newcommand{\icassp}[1][\scad]{\sca[#1]{icassp}\XS}
\newcommand{\spie}[1][\scad]{\sca[#1]{spie}\XS}
\newcommand{\gdr}[1][\scad]{\sca[#1]{gdr--prc~isis}\XS}
\newcommand{\rfia}[1][\scad]{\sca[#1]{rfia}\XS}
\newcommand{\eusipco}[1][\scad]{\sca[#1]{eusipco}\XS}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Ajout de famouss.tex
% modif le 25/5/2000 Phiphi
% GPInuts - Famous people - VIP
%
\newcommand{\beaunom}[4][0]{{\taille[#1]#2 \uppercase{#3}}%
{\sca[#1]{#4}}\XS}

%\newcommand{\MA}[1][\scad]{{\taille[#1]Marc \uppercase{A}}% 
%{\sca[#1]{llain}\XS}}
\newcommand{\MA}[1][\scad]{\beaunom[#1]{Marc}{A}{llain}}
\newcommand{\AB}[1][\scad]{\beaunom[#1]{Amandine}{B}{lanc}}
\newcommand{\ABF}[1][\scad]{\beaunom[#1]{Amandine}{B}{lanc~--~Fusco}}
\newcommand{\AC}[1][\scad]{\beaunom[#1]{Alain}{C}{oulais}}
\newcommand{\AH}[1][\scad]{\beaunom[#1]{Alain}{H}{erment}}
\newcommand{\AMD}[1][\scad]{\beaunom[#1]{Ali}{M}{ohammad--Djafari}}
\newcommand{\AR}[1][\scad]{\beaunom[#1]{Andrea}{R}{idolfi}}
\newcommand{\CH}[1][\scad]{\beaunom[#1]{Christian}{H}{einrich}}
\newcommand{\CS}[1][\scad]{\beaunom[#1]{Charles}{S}{oussen}}
\newcommand{\DLB}[1][\scad]{\beaunom[#1]{Denis}{L}{e Bihan}}
\newcommand{\FC}[1][\scad]{\beaunom[#1]{Fr\'ed\'eric}{C}{hampagnat}}
\newcommand{\FL}[1][\scad]{\beaunom[#1]{Franck}{L}{etimonier}}
\newcommand{\FV}[1][\scad]{\beaunom[#1]{Francisco}{V}{arela}}
\newcommand{\FDU}[1][\scad]{\beaunom[#1]{Fr\'ed\'eric}{D}{ublanchet}}
\newcommand{\GDE}[1][\scad]{\beaunom[#1]{Guy}{D}{emoment}}
\newcommand{\GLB}[1][\scad]{\beaunom[#1]{Guy Le}{B}{esnerais}}
\newcommand{\HC}[1][\scad]{\beaunom[#1]{Herv\'e}{C}{arfantan}}
\newcommand{\JFB}[1][\scad]{\beaunom[#1]{Jean--Fran\c{c}ois}{B}{ercher}}
\newcommand{\JFG}[1][\scad]{\beaunom[#1]{Jean--Fran\c{c}ois}{G}{iovannelli}}
\newcommand{\JFM}[1][\scad]{\beaunom[#1]{Jean--Fran\c{c}ois}{M}{angin}}
\newcommand{\JI}[1][\scad]{\beaunom[#1]{J\'er\^ome}{I}{dier}}
\newcommand{\JBP}[1][\scad]{\beaunom[#1]{Jean-Baptiste}{P}{oline}}
\newcommand{\MF}[1][\scad]{\beaunom[#1]{Marc}{F}{ayolle}}
\newcommand{\Mimi}[1][\scad]{\beaunom[#1]{Myriam}{F}{iani}}
\newcommand{\MN}[1][\scad]{\beaunom[#1]{Mila}{N}{ikolova}}
\newcommand{\PC}[1][\scad]{\beaunom[#1]{Philippe}{C}{iuciu}}
\newcommand{\LG}[1][\scad]{\beaunom[#1]{Line}{G}{arnero}}
\newcommand{\SB}[1][\scad]{\beaunom[#1]{St\'ephane}{B}{rette}}
\newcommand{\SBA}[1][\scad]{\beaunom[#1]{Sylvain}{B}{ailet}}
\newcommand{\RB}[1][\scad]{\beaunom[#1]{Redha}{B}{oubertakh}}
\newcommand{\TM}[1][\scad]{\beaunom[#1]{Thierry}{M}{artin}}
\newcommand{\VS}[1][\scad]{\beaunom[#1]{Vincent}{S}{amson}}
\newcommand{\YG}[1][\scad]{\beaunom[#1]{Yves}{G}{oussard}}
\newcommand{\KS}[1][\scad]{\beaunom[#1]{Ken}{S}{auer}}
\newcommand{\HS}[1][\scad]{\beaunom[#1]{Hichem}{S}{noussi}}

% Acronymes et raccourcis
%
\def\ATER{Attach\'e temporaire d'enseignement et de recherche}
\newcommand{\ater}[1][\scad]{\sca[#1]{ater}\xspace}
\def\ADDOC{Agir pour les Doctorants et les jeunes Docteurs\XS}
\newcommand{\addoc}[1][\scad]{\sca[#1]{addoc}\XS}

\def\CdO{Centre d'Orsay\XS}

\def\CEA{Commissariat � l'\'Enegie Atomique\XS}
\newcommand{\cea}[1][\scad]{\sca[#1]{cea}\XS}
\newcommand{\dam}[1][\scad]{\sca[#1]{dam}\XS}
\def\DRM{D\'epartement de Recherche M\'edicale\XS}
\newcommand{\drm}[1][\scad]{\sca[#1]{drm}\XS}
\def\DSV{Direction des Sciences du Vivant\XS}
\newcommand{\dsv}[1][\scad]{\sca[#1]{dsv}\XS}
\newcommand{\leti}[1][\scad]{\sca[#1]{leti}\XS}
\def\SHFJ{Service Hospitalier Fr�d�ric Joliot\XS}
\newcommand{\shfj}[1][\scad]{\sca[#1]{shfj}\XS}
\def\UNAF{Unit\'e de Neuroimagerie Anatomo Foncxtionnelle\XS}
\newcommand{\unaf}[1][\scad]{\sca[#1]{unaf}\XS}


\newcommand{\chu}[1][\scad]{\sca[#1]{chu}\XS}
\def\CHU{Centre Hospitalier Universitaire\XS}
\def\salpe{Salp�tri�re\XS}
\def\hsalpe{H�pital de la Salp�tri�re\XS}
\def\pisalpe{Piti�-Salp�tri�re\XS}
\def\gpisalpe{Groupe Piti�-Salp�tri�re\XS}

\def\CNRS{Centre National de la Recherche Scientifique\XS}
\newcommand{\cnrs}[1][\scad]{\sca[#1]{cnrs}\XS}

\newcommand{\edf}[1][\scad]{\sca[#1]{edf}\XS}
\def\EDF{\'Electricit� de France\XS}

\def\ENSTA{\'Ecole Nationale Sup\'erieure de Techniques Avanc\'ees\XS}
\newcommand{\ensta}[1][\scad]{\sca[#1]{ensta}\XS}
\def\ESIEA{\'Ecole Sup�rieure d'Informatique \'Electronique Automatique\XS}
\newcommand{\esiea}[1][\scad]{\sca[#1]{esiea}\XS}
\newcommand{\ensea}[1][\scad]{\sca[#1]{ensea}\XS}


\def\GPI{Groupe Probl\`emes Inverses\XS}
\newcommand{\gpi}[1][\scad]{\sca[#1]{gpi}\XS}

\def\INSERM{Institut National pour la Sant\'e et la Recherche M\'edicale\XS}
\newcommand{\inserm}[1][\scad]{\sca[#1]{inserm}\XS}

\def\CNAM{Conservatoire National des Arts et M�tiers\XS}
\newcommand{\cnam}[1][\scad]{\sca[#1]{cnam}\XS}

\def\INRIA{Institut National de Recherche et Informatique et Automatique\XS}
\newcommand{\inria}[1][\scad]{\sca[#1]{inria}\XS}

\def\IAS{Institut d'Astrophysique Spatiale\XS}
\newcommand{\ias}[1][\scad]{\sca[#1]{ias}\XS}

\newcommand{\ipsn}[1][\scad]{\sca[#1]{ipsn}\XS}
\def\IPSN{Institut de Protection et de Suret� Nucl�aire\XS}

\def\LSS{Laboratoire des Signaux et Syst\`emes\XS}
\newcommand{\lss}[1][\scad]{\sca[#1]{l{\footnotesize 2}s}\XS}

\def\LIMSI{Laboratoire d'Informatique pour la M�canique et les Sciences de l'Ing�nieur\XS}
\newcommand{\limsi}[1][\scad]{\sca[#1]{limsi-cnrs}\XS}

\def\ONERA{Office National d'\'Etudes et de Recherches A\'erospatiales\XS}
\newcommand{\onera}[1][\scad]{\sca[#1]{on\'era}\XS}

\def\MDC{Ma\^\i tre de conf\'erences\XS}
\def\MDCs{Ma\^\i tres de conf\'erences\XS}
\newcommand{\mdc}[1][\scad]{\sca[#1]{mdc}\XS}

\newcommand{\UND}[1][\scad]{Universit� de Notre Dame, \sca[#1]{usa}\XS}

\def\UPS{Universit\'e Paris-Sud\XS}
\newcommand{\ups}[1][\scad]{\sca[#1]{ups}\XS}
\newcommand{\upxi}[1][\scad]{\sca[#1]{upxi}\XS}

% Unites Thomson
\newcommand{\thomair}[1][\scad]{\sca[#1]{Thomson-csf Airsys}\XS}
\newcommand{\oscar}[1][\scad]{\sca[#1]{Oscar}\XS}
\newcommand{\thomrcm}[1][\scad]{\sca[#1]{Thomson-rcm}\XS}

% Unite propre de recherche
\newcommand{\upr}[1][\scad]{\sca[#1]{upr}\XS}
% LENA, lena upr640,...
\newcommand{\uprlen}[1][\scad]{\sca[#1]{upr}{\footnotesize 640}\XS}
\def\LENA{Laboratoire d'Enc�phalographie et de Neurophysiologie Appliqu�e\XS}
\newcommand{\lena}[1][\scad]{\sca[#1]{lena}\XS}
% Nous
\def\GsY{Gif--sur--Yvette\XS}
\newcommand{\ESE}[1][\scad]{\sca[#1]{sup\'elec}\XS}

\def\adrshort{\ESE, Plateau de Moulon, 91192 Gif--sur--Yvette Cedex\XS}
%\def\adresse{\ESE, Plateau de Moulon, 91192 Gif--sur--Yvette Cedex, France\XS}
\newcommand{\hiercea}[1][\scad]{\dsv[#1]/\drm[#1]/\shfj[#1]\XS}

\newcommand{\adresse}[1][\scad]{\ESE[#1], Plateau de Moulon, 91192 Gif--sur--Yvette Cedex, France\XS}
\newcommand{\adresscea}[1][\scad]{4 Place du G�n�ral Leclerc, 91406 Orsay Cedex, France\XS}
\newcommand{\tutelle}[1][\scad]{\cnrs[#1]~--~\ESE[#1]~--~\ups[#1]}
%\newcommand{\tutelle}[1][\scad]{\sca[#1]{Cnrs~--~Sup\'elec~--~Ups}}
\def\ALSS{\LSS~(\tutelle)\\\adresse}
\def\ALSSun{\LSS (\tutelle) \adresse}
%


% ---------------------------------------------------- 
% Modele d'en-tete par A. Mohammad-Djafari et J. Idier 
% ---------------------------------------------------- 
%
\def\helvnormal#1{{\fontfamily{phv}\fontsize{11}{14pt}\selectfont #1}}
\def\helvfoot  #1{{\fontfamily{phv}\fontsize{9}{14pt} \selectfont #1}}
\def\helvscript#1{{\fontfamily{phv}\fontsize{8}{14pt} \selectfont #1}}
%
\newcommand{\entete}[5][Nom.Pr\'enom]{
%%%%%%\def\entete#1#2#3#4#5{%
\helvscript{\renewcommand{\arraystretch}{.8}
\begin{tabular}{c} Sup�lec
\\--------\end{tabular} \hfill
\begin{tabular}{c}Centre national de la recherche scientifique          \\
--------\end{tabular} \hfill
\begin{tabular}{c}\UPS  \\--------\end{tabular}} \\[-.4cm]%
%
\begin{center}\helvnormal{\textbf{LABORATOIRE DES SIGNAUX \& SYST\`EMES}}\\%
\helvfoot{Unit\'e mixte de recherche n$^{\rm o}$ 8506\\%
Sup\'elec, plateau de Moulon, 
3 rue Joliot-Curie, 91192 \sca[-3]{Gif--sur--Yvette} Cedex (France)\\%
T\'el\'ephone\,: 01 69 85 17 12 --- 
T\'el\'ecopie\,: 01 69 85 17 65 --- 
Courriel\,: {#1}@lss.supelec.fr}%
\\[0.5cm]\end{center}% 
\begin{tabular}{p{8.5cm}l}%
\helvscript{V/R\'ef.\,: #2} & \helvscript{\sca[-3]{Gif}, le} #5\\%
\helvscript{N/R\'ef.\,: #3} \\%
\helvscript{Objet\,: #4}%
\end{tabular}
} 

\newcommand{\inhead}[5][Name.Surname]{
%%%%%%\def\entete#1#2#3#4#5{%
\helvscript{\renewcommand{\arraystretch}{.8}
\begin{tabular}{c} Sup�lec
\\--------\end{tabular} \hfill
\begin{tabular}{c}Centre national de la recherche scientifique  \\
--------\end{tabular} \hfill
\begin{tabular}{c}\UPS  \\--------\end{tabular}} \\[-.4cm]%
%
\begin{center}\helvnormal{\textbf{LABORATOIRE DES SIGNAUX \& SYST\`EMES}}\\%
\helvfoot{Unit\'e mixte de recherche n$^{\rm o}$ 8506\\%
Sup\'elec, plateau de Moulon, 
3 rue Joliot-Curie, 91192 \sca[-3]{Gif--sur--Yvette} Cedex (France)\\%
Telephone: 01 69 85 17 12 --- 
Fax: 01 69 85 17 65 --- 
E-mail: {#1}@lss.supelec.fr}%
\\[0.5cm]\end{center}% 
\begin{tabular}{p{8.5cm}l}%
\helvscript{Y/Ref.: #2} & \helvscript{\sca[-3]{Gif}, } #5\\%
\helvscript{O/Ref.: #3} \\%
\helvscript{Subject: #4}%
\end{tabular}
} 



==> alphabet.tex <==
% Document LaTeX        Auteur : Guy Le Besnerais       Date : 25/05/94
% Modification : J.-F. Gio      (15/09/95)
%                               J.I. (format Latex 2e, taille adaptative 22/03/99)
%                                    (fonte blackboard 27/08/99)

% Objet : Definitions compactes d'alphabets pour ecriture en Math
% b pour bold italique : \Ab
% v pour bold droit : \Av
% D pour droit : \AD
% c pour cursif : \Ac
% bb pour blackboard : \Abb
% Capitale pour capitale : \Lambda

\typeout{\space}
\typeout{\space\space\space\space Fichier 'alphabet.tex' -- LSS 1994/95/99}
\typeout{\space\space\space\space (necessite les packages xspace, amsmath, bbm)}
\typeout{\space}

\RequirePackage{amsmath}
\RequirePackage{xspace}
\RequirePackage{bbm}
\RequirePackage{oldgerm}		% 04.06.2003   Pour les alphabet Gauthiques

%-------------------------------------------

% DEFINITIONS PRELIMINAIRES 

\def\XS{\xspace}
\DeclareMathAlphabet{\mathb}{OML}{cmm}{b}{it}
\def\sbm#1{\ensuremath{\mathb{#1}}}                % Style gras italique (necessite amsmath)           
%
\def\sbmm#1{\ensuremath{\boldsymbol{#1}}}          % Style gras italique (necessite amsmath)           
\def\sdm#1{\ensuremath{\mathrm{#1}}}               % Style droit en math
\def\sbv#1{\ensuremath{\mathbf{#1}}}               % Style gras droit
\def\scu#1{\ensuremath{\mathcal{#1\XS}}}           % Style cursif
\def\scb#1{\ensuremath{\boldsymbol{\mathcal{#1}}}} % Style gras cursif
\def\sbl#1{\ensuremath{\mathbbm{#1}}}              % Style blackboard (necessite bbm)

%-------------------------------------------

% ALPHABET GRAS ITALIQUE, taille adaptative

\def\Ab{{\sbm{A}}\XS}  \def\ab{{\sbm{a}}\XS}
\def\Bb{{\sbm{B}}\XS}  \def\bb{{\sbm{b}}\XS}
\def\Cb{{\sbm{C}}\XS}  \def\cb{{\sbm{c}}\XS}
\def\Db{{\sbm{D}}\XS}  \def\db{{\sbm{d}}\XS}
\def\Eb{{\sbm{E}}\XS}  \def\eb{{\sbm{e}}\XS}
\def\Fb{{\sbm{F}}\XS}  \def\fb{{\sbm{f}}\XS}
\def\Gb{{\sbm{G}}\XS}  \def\gb{{\sbm{g}}\XS}
\def\Hb{{\sbm{H}}\XS}  \def\hb{{\sbm{h}}\XS}
\def\Ib{{\sbm{I}}\XS}  \def\ib{{\sbm{i}}\XS}
\def\Jb{{\sbm{J}}\XS}  \def\jb{{\sbm{j}}\XS}
\def\Kb{{\sbm{K}}\XS}  \def\kb{{\sbm{k}}\XS}
\def\Lb{{\sbm{L}}\XS}  \def\lb{{\sbm{l}}\XS}
\def\Mb{{\sbm{M}}\XS}  \def\mb{{\sbm{m}}\XS}
\def\Nb{{\sbm{N}}\XS}  \def\nb{{\sbm{n}}\XS}
\def\Ob{{\sbm{O}}\XS}  \def\ob{{\sbm{o}}\XS}
\def\Pb{{\sbm{P}}\XS}  \def\pb{{\sbm{p}}\XS}
\def\Qb{{\sbm{Q}}\XS}  \def\qb{{\sbm{q}}\XS}
\def\Rb{{\sbm{R}}\XS}  \def\rb{{\sbm{r}}\XS}
\def\Sb{{\sbm{S}}\XS}  \def\sb{{\sbm{s}}\XS}
\def\Tb{{\sbm{T}}\XS}  \def\tb{{\sbm{t}}\XS}
\def\Ub{{\sbm{U}}\XS}  \def\ub{{\sbm{u}}\XS}
\def\Vb{{\sbm{V}}\XS}  \def\vb{{\sbm{v}}\XS}
\def\Wb{{\sbm{W}}\XS}  \def\wb{{\sbm{w}}\XS}
\def\Xb{{\sbm{X}}\XS}  \def\xb{{\sbm{x}}\XS}
\def\Yb{{\sbm{Y}}\XS}  \def\yb{{\sbm{y}}\XS}
\def\Zb{{\sbm{Z}}\XS}  \def\zb{{\sbm{z}}\XS}


% ALPHABET CURSIF MAJUSCULE, taille adaptative
% Cursif,               % Cursif gras

\def\Ac{{\scu{A}}\XS}   \def\Acb{{\scb{A}}\XS}
\def\Bc{{\scu{B}}\XS}   \def\Bcb{{\scb{B}}\XS}
\def\Cc{{\scu{C}}\XS}   \def\Ccb{{\scb{C}}\XS}
\def\Dc{{\scu{D}}\XS}   \def\Dcb{{\scb{D}}\XS}
\def\Ec{{\scu{E}}\XS}   \def\Ecb{{\scb{E}}\XS}
\def\Fc{{\scu{F}}\XS}   \def\Fcb{{\scb{F}}\XS}
\def\Gc{{\scu{G}}\XS}   \def\Gcb{{\scb{G}}\XS}
\def\Hc{{\scu{H}}\XS}   \def\Hcb{{\scb{H}}\XS}
\def\Ic{{\scu{I}}\XS}   \def\Icb{{\scb{I}}\XS}
\def\Jc{{\scu{J}}\XS}   \def\Jcb{{\scb{J}}\XS}
\def\Kc{{\scu{K}}\XS}   \def\Kcb{{\scb{K}}\XS}
\def\Lc{{\scu{L}}\XS}   \def\Lcb{{\scb{L}}\XS}
\def\Mc{{\scu{M}}\XS}   \def\Mcb{{\scb{M}}\XS}
\def\Nc{{\scu{N}}\XS}   \def\Ncb{{\scb{N}}\XS}
\def\Oc{{\scu{O}}\XS}   \def\Ocb{{\scb{O}}\XS}
\def\Pc{{\scu{P}}\XS}   \def\Pcb{{\scb{P}}\XS}
\def\Qc{{\scu{Q}}\XS}   \def\Qcb{{\scb{Q}}\XS}
\def\Rc{{\scu{R}}\XS}   \def\Rcb{{\scb{R}}\XS}
\def\Sc{{\scu{S}}\XS}   \def\Scb{{\scb{S}}\XS}
\def\Tc{{\scu{T}}\XS}   \def\Tcb{{\scb{T}}\XS}
\def\Uc{{\scu{U}}\XS}   \def\Ucb{{\scb{U}}\XS}
\def\Vc{{\scu{V}}\XS}   \def\Vcb{{\scb{V}}\XS}
\def\Wc{{\scu{W}}\XS}   \def\Wcb{{\scb{W}}\XS}
\def\Xc{{\scu{X}}\XS}   \def\Xcb{{\scb{X}}\XS}
\def\Yc{{\scu{Y}}\XS}   \def\Ycb{{\scb{Y}}\XS}
\def\Zc{{\scu{Z}}\XS}   \def\Zcb{{\scb{Z}}\XS}


% ALPHABET DROIT EN MATHS, taille adaptative

\def\AD{{\sdm{A}}\XS}  \def\aD{{\sdm{a}}\XS}
\def\BD{{\sdm{B}}\XS}  \def\bD{{\sdm{b}}\XS}
\def\CD{{\sdm{C}}\XS}  \def\cD{{\sdm{c}}\XS}
\def\DD{{\sdm{D}}\XS}  \def\dD{{\sdm{d}}\XS}
\def\ED{{\sdm{E}}\XS}  \def\eD{{\sdm{e}}\XS}
\def\FD{{\sdm{F}}\XS}  \def\fD{{\sdm{f}}\XS}
\def\GD{{\sdm{G}}\XS}  \def\gD{{\sdm{g}}\XS}
\def\HD{{\sdm{H}}\XS}  \def\hD{{\sdm{h}}\XS}
\def\ID{{\sdm{I}}\XS}  \def\iD{{\sdm{i}}\XS}
\def\JD{{\sdm{J}}\XS}  \def\jD{{\sdm{j}}\XS}
\def\KD{{\sdm{K}}\XS}  \def\kD{{\sdm{k}}\XS}
\def\LD{{\sdm{L}}\XS}  \def\lD{{\sdm{l}}\XS}
\def\MD{{\sdm{M}}\XS}  \def\mD{{\sdm{m}}\XS}
\def\ND{{\sdm{N}}\XS}  \def\nD{{\sdm{n}}\XS}
\def\OD{{\sdm{O}}\XS}  \def\oD{{\sdm{o}}\XS}
\def\PD{{\sdm{P}}\XS}  \def\pD{{\sdm{p}}\XS}
\def\QD{{\sdm{Q}}\XS}  \def\qD{{\sdm{q}}\XS}
\def\RD{{\sdm{R}}\XS}  \def\rD{{\sdm{r}}\XS}
\def\SD{{\sdm{S}}\XS}  \def\sD{{\sdm{s}}\XS}
\def\TD{{\sdm{T}}\XS}  \def\tD{{\sdm{t}}\XS}
\def\UD{{\sdm{U}}\XS}  \def\uD{{\sdm{u}}\XS}
\def\VD{{\sdm{V}}\XS}  \def\vD{{\sdm{D}}\XS}
\def\WD{{\sdm{W}}\XS}  \def\wD{{\sdm{w}}\XS}
\def\XD{{\sdm{X}}\XS}  \def\xD{{\sdm{x}}\XS}
\def\YD{{\sdm{Y}}\XS}  \def\yD{{\sdm{y}}\XS}
\def\ZD{{\sdm{Z}}\XS}  \def\zD{{\sdm{z}}\XS}


% ALPHABET GRAS DROIT, taille adaptative

\def\Av{{\sbv{A}}\XS}  \def\av{{\sbv{a}}\XS}
\def\Bv{{\sbv{B}}\XS}  \def\bv{{\sbv{b}}\XS}
\def\Cv{{\sbv{C}}\XS}  \def\cv{{\sbv{c}}\XS}
\def\Dv{{\sbv{D}}\XS}  \def\dv{{\sbv{d}}\XS}
\def\Ev{{\sbv{E}}\XS}  \def\ev{{\sbv{e}}\XS}
\def\Fv{{\sbv{F}}\XS}  \def\fv{{\sbv{f}}\XS}
\def\Gv{{\sbv{G}}\XS}  \def\gv{{\sbv{g}}\XS}
\def\Hv{{\sbv{H}}\XS}  \def\hv{{\sbv{h}}\XS}
\def\Iv{{\sbv{I}}\XS}  \def\iv{{\sbv{i}}\XS}
\def\Jv{{\sbv{J}}\XS}  \def\jv{{\sbv{j}}\XS}
\def\Kv{{\sbv{K}}\XS}  \def\kv{{\sbv{k}}\XS}
\def\Lv{{\sbv{L}}\XS}  \def\lv{{\sbv{l}}\XS}
\def\Mv{{\sbv{M}}\XS}  \def\mv{{\sbv{m}}\XS}
\def\Nv{{\sbv{N}}\XS}  \def\nv{{\sbv{n}}\XS}
\def\Ov{{\sbv{O}}\XS}  \def\ov{{\sbv{o}}\XS}
\def\Pv{{\sbv{P}}\XS}  \def\pv{{\sbv{p}}\XS}
\def\Qv{{\sbv{Q}}\XS}  \def\qv{{\sbv{q}}\XS}
\def\Rv{{\sbv{R}}\XS}  \def\rv{{\sbv{r}}\XS}
\def\Sv{{\sbv{S}}\XS}  \def\sv{{\sbv{s}}\XS}
\def\Tv{{\sbv{T}}\XS}  \def\tv{{\sbv{t}}\XS}
\def\Uv{{\sbv{U}}\XS}  \def\uv{{\sbv{u}}\XS}
\def\Vv{{\sbv{V}}\XS}  \def\vv{{\sbv{v}}\XS}
\def\Wv{{\sbv{W}}\XS}  \def\wv{{\sbv{w}}\XS}
\def\Xv{{\sbv{X}}\XS}  \def\xv{{\sbv{x}}\XS}
\def\Yv{{\sbv{Y}}\XS}  \def\yv{{\sbv{y}}\XS}
\def\Zv{{\sbv{Z}}\XS}  \def\zv{{\sbv{z}}\XS}


% Nouveau (08/99) : ALPHABET BLACKBOARD, taille adaptative

\def\Abb{{\sbl{A}}\XS}  \def\abb{{\sbl{a}}\XS}
\def\Bbb{{\sbl{B}}\XS}  \def\bbb{{\sbl{b}}\XS}
\def\Cbb{{\sbl{C}}\XS}  \def\cbb{{\sbl{c}}\XS}
\def\Dbb{{\sbl{D}}\XS}  \def\dbb{{\sbl{d}}\XS}
\def\Ebb{{\sbl{E}}\XS}  \def\ebb{{\sbl{e}}\XS}
\def\Fbb{{\sbl{F}}\XS}  \def\fbb{{\sbl{f}}\XS}
\def\Gbb{{\sbl{G}}\XS}  \def\gbb{{\sbl{g}}\XS}
\def\Hbb{{\sbl{H}}\XS}  \def\hbb{{\sbl{h}}\XS}
\def\Ibb{{\sbl{I}}\XS}  \def\ibb{{\sbl{i}}\XS}
\def\Jbb{{\sbl{J}}\XS}  \def\jbb{{\sbl{j}}\XS}
\def\Kbb{{\sbl{K}}\XS}  \def\kbb{{\sbl{k}}\XS}
\def\Lbb{{\sbl{L}}\XS}  \def\lbb{{\sbl{l}}\XS}
\def\Mbb{{\sbl{M}}\XS}  \def\mbb{{\sbl{m}}\XS}
\def\Nbb{{\sbl{N}}\XS}  \def\nbb{{\sbl{n}}\XS}
\def\Obb{{\sbl{O}}\XS}  \def\obb{{\sbl{o}}\XS}
\def\Pbb{{\sbl{P}}\XS}  \def\pbb{{\sbl{p}}\XS}
\def\Qbb{{\sbl{Q}}\XS}  \def\qbb{{\sbl{q}}\XS}
\def\Rbb{{\sbl{R}}\XS}  \def\rbb{{\sbl{r}}\XS}
\def\Sbb{{\sbl{S}}\XS}  \def\sbb{{\sbl{s}}\XS}
\def\Tbb{{\sbl{T}}\XS}  \def\tbb{{\sbl{t}}\XS}
\def\Ubb{{\sbl{U}}\XS}  \def\ubb{{\sbl{u}}\XS}
\def\Vbb{{\sbl{V}}\XS}  \def\vbb{{\sbl{v}}\XS}
\def\Wbb{{\sbl{W}}\XS}  \def\wbb{{\sbl{w}}\XS}
\def\Xbb{{\sbl{X}}\XS}  \def\xbb{{\sbl{x}}\XS}
\def\Ybb{{\sbl{Y}}\XS}  \def\ybb{{\sbl{y}}\XS}
\def\Zbb{{\sbl{Z}}\XS}  \def\zbb{{\sbl{z}}\XS}

% ALPHABET GRAS et Chapeau
\def\Abh{\hat{{\sbm{A}}}\XS}  \def\abh{\hat{{\sbm{a}}}\XS}
\def\Bbh{\hat{{\sbm{B}}}\XS}  \def\bbh{\hat{{\sbm{b}}}\XS}
\def\Cbh{\hat{{\sbm{C}}}\XS}  \def\cbh{\hat{{\sbm{c}}}\XS}
\def\Dbh{\hat{{\sbm{D}}}\XS}  \def\dbh{\hat{{\sbm{d}}}\XS}
\def\Ebh{\hat{{\sbm{E}}}\XS}  \def\ebh{\hat{{\sbm{e}}}\XS}
\def\Fbh{\hat{{\sbm{F}}}\XS}  \def\fbh{\hat{{\sbm{f}}}\XS}
\def\Gbh{\hat{{\sbm{G}}}\XS}  \def\gbh{\hat{{\sbm{g}}}\XS}
\def\Hbh{\hat{{\sbm{H}}}\XS}  \def\hbh{\hat{{\sbm{h}}}\XS}
\def\Ibh{\hat{{\sbm{I}}}\XS}  \def\ibh{\hat{{\sbm{i}}}\XS}
\def\Jbh{\hat{{\sbm{J}}}\XS}  \def\jbh{\hat{{\sbm{j}}}\XS}
\def\Kbh{\hat{{\sbm{K}}}\XS}  \def\kbh{\hat{{\sbm{k}}}\XS}
\def\Lbh{\hat{{\sbm{L}}}\XS}  \def\lbh{\hat{{\sbm{l}}}\XS}
\def\Mbh{\hat{{\sbm{M}}}\XS}  \def\mbh{\hat{{\sbm{m}}}\XS}
\def\Nbh{\hat{{\sbm{N}}}\XS}  \def\nbh{\hat{{\sbm{n}}}\XS}
\def\Obh{\hat{{\sbm{O}}}\XS}  \def\obh{\hat{{\sbm{o}}}\XS}
\def\Pbh{\hat{{\sbm{P}}}\XS}  \def\pbh{\hat{{\sbm{p}}}\XS}
\def\Qbh{\hat{{\sbm{Q}}}\XS}  \def\qbh{\hat{{\sbm{q}}}\XS}
\def\Rbh{\hat{{\sbm{R}}}\XS}  \def\rbh{\hat{{\sbm{r}}}\XS}
\def\Sbh{\hat{{\sbm{S}}}\XS}  \def\sbh{\hat{{\sbm{s}}}\XS}
\def\Tbh{\hat{{\sbm{T}}}\XS}  \def\tbh{\hat{{\sbm{t}}}\XS}
\def\Ubh{\hat{{\sbm{U}}}\XS}  \def\ubh{\hat{{\sbm{u}}}\XS}
\def\Vbh{\hat{{\sbm{V}}}\XS}  \def\vbh{\hat{{\sbm{v}}}\XS}
\def\Wbh{\hat{{\sbm{W}}}\XS}  \def\wbh{\hat{{\sbm{w}}}\XS}
\def\Xbh{\hat{{\sbm{X}}}\XS}  \def\xbh{\hat{{\sbm{x}}}\XS}
\def\Ybh{\hat{{\sbm{Y}}}\XS}  \def\ybh{\hat{{\sbm{y}}}\XS}
\def\Zbh{\hat{{\sbm{Z}}}\XS}  \def\zbh{\hat{{\sbm{z}}}\XS}

\def\alphabh      {\hat{{\sbmm{\alpha}}}\XS}
\def\betabh       {\hat{{\sbmm{\beta}}}\XS}
\def\gammabh      {\hat{{\sbmm{\gamma}}}\XS}      \def\Gammabh    {\hat{{\sbmm{\Gamma}}}\XS}
\def\deltabh      {\hat{{\sbmm{\delta}}}\XS}      \def\Deltabh    {\hat{{\sbmm{\Delta}}}\XS}
\def\epsilonbh    {\hat{{\sbmm{\epsilon}}}\XS}
\def\varepsilonbh {\hat{{\sbmm{\varepsilon}}}\XS}
\def\etabh        {\hat{{\sbmm{\eta}}}\XS}
\def\thetabh      {\hat{{\sbmm{\theta}}}\XS}      \def\Thetabh    {\hat{{\sbmm{\Theta}}}\XS}
\def\varthetabh   {\hat{{\sbmm{\vartheta}}}\XS}
\def\iotabh       {\hat{{\sbmm{\iota}}}\XS}
\def\kappabh      {\hat{{\sbmm{\kappa}}}\XS}
\def\varkappabh   {\hat{{\sbmm{\varkappa}}}\XS}
\def\lambdabh     {\hat{{\sbmm{\lambda}}}\XS}     \def\Lambdabh   {\hat{{\sbmm{\Lambda}}}\XS}
\def\mubh         {\hat{{\sbmm{\mu}}}\XS}
\def\nubh         {\hat{{\sbmm{\nu}}}\XS}
\def\xibh         {\hat{{\sbmm{\xi}}}\XS}         \def\Xibh       {\hat{{\sbmm{\Xi}}}\XS}
\def\pibh         {\hat{{\sbmm{\pi}}}\XS}         \def\Pibh       {\hat{{\sbmm{\Pi}}}\XS}
\def\varpibh      {\hat{{\sbmm{\varpi}}}\XS}
\def\rhobh        {\hat{{\sbmm{\rho}}}\XS}
\def\varrhobh     {\hat{{\sbmm{\varrho}}}\XS}
\def\sigmabh      {\hat{{\sbmm{\sigma}}}\XS}      \def\Sigmabh    {\hat{{\sbmm{\Sigma}}}\XS}
\def\varsigmabh   {\hat{{\sbmm{\varsigma}}}\XS}   \def\Varsigmabh {\hat{{\sbmm{\Varsigma}}}\XS}
\def\phibh        {\hat{{\sbmm{\phi}}}\XS}        \def\Phibh      {\hat{{\sbmm{\Phi}}}\XS}
\def\varphibh     {\hat{{\sbmm{\varphi}}}\XS}
\def\chibh        {\hat{{\sbmm{\chi}}}\XS}
\def\psibh        {\hat{{\sbmm{\psi}}}\XS}        \def\Psibh      {\hat{{\sbmm{\Psi}}}\XS}
\def\omegabh      {\hat{{\sbmm{\omega}}}\XS}      \def\Omegabh    {\hat{{\sbmm{\Omega}}}\XS}
\def\taubh        {\hat{{\sbmm{\tau}}}\XS}
\def\upsilonbh    {\hat{{\sbmm{\upsilon}}}\XS}   \def\Upsilonbh  {\hat{{\sbmm{\Upsilon}}}\XS}
\def\zetabh       {\hat{{\sbmm{\zeta}}}\XS}





% ALPHABET GREC GRAS italique, taille adaptative

\def\alphab      {{\sbmm{\alpha}}\XS}
\def\betab       {{\sbmm{\beta}}\XS}
\def\gammab      {{\sbmm{\gamma}}\XS}      \def\Gammab    {{\sbmm{\Gamma}}\XS}
\def\deltab      {{\sbmm{\delta}}\XS}      \def\Deltab    {{\sbmm{\Delta}}\XS}
\def\epsilonb    {{\sbmm{\epsilon}}\XS}
\def\varepsilonb {{\sbmm{\varepsilon}}\XS}
\def\etab        {{\sbmm{\eta}}\XS}
\def\thetab      {{\sbmm{\theta}}\XS}      \def\Thetab    {{\sbmm{\Theta}}\XS}
\def\varthetab   {{\sbmm{\vartheta}}\XS}
\def\iotab       {{\sbmm{\iota}}\XS}
\def\kappab      {{\sbmm{\kappa}}\XS}
\def\varkappab   {{\sbmm{\varkappa}}\XS}
\def\lambdab     {{\sbmm{\lambda}}\XS}     \def\Lambdab   {{\sbmm{\Lambda}}\XS}
\def\mub         {{\sbmm{\mu}}\XS}
\def\nub         {{\sbmm{\nu}}\XS}
\def\xib         {{\sbmm{\xi}}\XS}         \def\Xib       {{\sbmm{\Xi}}\XS}
\def\pib         {{\sbmm{\pi}}\XS}         \def\Pib       {{\sbmm{\Pi}}\XS}
\def\varpib      {{\sbmm{\varpi}}\XS}
\def\rhob        {{\sbmm{\rho}}\XS}
\def\varrhob     {{\sbmm{\varrho}}\XS}
\def\sigmab      {{\sbmm{\sigma}}\XS}      \def\Sigmab    {{\sbmm{\Sigma}}\XS}
\def\varsigmab   {{\sbmm{\varsigma}}\XS}   \def\Varsigmab {{\sbmm{\Varsigma}}\XS}
\def\phib        {{\sbmm{\phi}}\XS}        \def\Phib      {{\sbmm{\Phi}}\XS}
\def\varphib     {{\sbmm{\varphi}}\XS}
\def\chib        {{\sbmm{\chi}}\XS}
\def\psib        {{\sbmm{\psi}}\XS}        \def\Psib      {{\sbmm{\Psi}}\XS}
\def\omegab      {{\sbmm{\omega}}\XS}      \def\Omegab    {{\sbmm{\Omega}}\XS}
\def\taub        {{\sbmm{\tau}}\XS}
\def\upsilonb    {{\sbmm{\upsilon}}\XS}   \def\Upsilonb  {{\sbmm{\Upsilon}}\XS}
\def\zetab       {{\sbmm{\zeta}}\XS}


% CHIFFRES
% Gras et Blackboard, taille adaptative

\def\zerob   {{\sbv{0}}\XS}        \def\zerobb   {{\sbl{O}}\XS}
\def\unb     {{\sbv{1}}\XS}        \def\unbb     {{\sbl{1}}\XS}
\def\deuxb   {{\sbv{2}}\XS}        \def\deuxbb   {{\sbl{2}}\XS}
\def\troisb  {{\sbv{3}}\XS}        \def\troisbb  {{\sbl{3}}\XS}
\def\quatreb {{\sbv{4}}\XS}        \def\quatrebb {{\sbl{4}}\XS}
\def\cinqb   {{\sbv{5}}\XS}        \def\cinqbb   {{\sbl{5}}\XS}
\def\sixb    {{\sbv{6}}\XS}        \def\sixbb    {{\sbl{6}}\XS}
\def\septb   {{\sbv{7}}\XS}        \def\septbb   {{\sbl{7}}\XS}
\def\huitb   {{\sbv{8}}\XS}        \def\huitbb   {{\sbl{8}}\XS}
\def\neufb   {{\sbv{9}}\XS}        \def\neufbb   {{\sbl{9}}\XS}


% QUELQUES ENSEMBLES

\def\eC{\Cbb}
\def\eE{\Ebb}
\def\eN{\Nbb}
\def\eQ{\Qbb}
\def\eR{\Rbb}
\def\eZ{\Zbb}

% ALPHABET GAUTHIQUES  04.06.2003  M.M. ICHIR

\def\Ag{{\textgoth{A}}\XS}  \def\ag{{\textgoth{a}}\XS}
\def\Bg{{\textgoth{B}}\XS}  \def\bg{{\textgoth{b}}\XS}
\def\Cg{{\textgoth{C}}\XS}  \def\cg{{\textgoth{c}}\XS}
\def\Dg{{\textgoth{D}}\XS}  \def\dg{{\textgoth{d}}\XS}
\def\Eg{{\textgoth{E}}\XS}  \def\eg{{\textgoth{e}}\XS}
\def\Fg{{\textgoth{F}}\XS}  \def\fg{{\textgoth{f}}\XS}
\def\Gg{{\textgoth{G}}\XS}  \def\gg{{\textgoth{g}}\XS}
\def\Hg{{\textgoth{H}}\XS}  \def\hg{{\textgoth{h}}\XS}
\def\Ig{{\textgoth{I}}\XS}  \def\ig{{\textgoth{i}}\XS}
\def\Jg{{\textgoth{J}}\XS}  \def\jg{{\textgoth{j}}\XS}
\def\Kg{{\textgoth{K}}\XS}  \def\kg{{\textgoth{k}}\XS}
\def\Lg{{\textgoth{L}}\XS}  \def\lg{{\textgoth{l}}\XS}
\def\Mg{{\textgoth{M}}\XS}  \def\mg{{\textgoth{m}}\XS}
\def\Ng{{\textgoth{N}}\XS}  \def\ng{{\textgoth{n}}\XS}
\def\Og{{\textgoth{O}}\XS}  \def\og{{\textgoth{o}}\XS}
\def\Pg{{\textgoth{P}}\XS}  \def\pg{{\textgoth{p}}\XS}
\def\Qg{{\textgoth{Q}}\XS}  \def\qg{{\textgoth{q}}\XS}
\def\Rg{{\textgoth{R}}\XS}  \def\rg{{\textgoth{r}}\XS}
\def\Sg{{\textgoth{S}}\XS}  \def\sg{{\textgoth{s}}\XS}
\def\Tg{{\textgoth{T}}\XS}  \def\tg{{\textgoth{t}}\XS}
\def\Ug{{\textgoth{U}}\XS}  \def\ug{{\textgoth{u}}\XS}
\def\Vg{{\textgoth{V}}\XS}  \def\vg{{\textgoth{v}}\XS}
\def\Wg{{\textgoth{W}}\XS}  \def\wg{{\textgoth{w}}\XS}
\def\Xg{{\textgoth{X}}\XS}  \def\xg{{\textgoth{x}}\XS}
\def\Yg{{\textgoth{Y}}\XS}  \def\yg{{\textgoth{y}}\XS}
\def\Zg{{\textgoth{Z}}\XS}  \def\zg{{\textgoth{z}}\XS}

